Optimizing Lead Time in Fall Detection for a Planar Bipedal Robot

For legged robots to operate in complex terrains, they must be robust to the disturbances and uncertainties they encounter. This paper contributes to enhancing robustness through the design of fall detection/prediction algorithms that will provide sufficient lead time for corrective motions to be taken. Falls can be caused by abrupt (fast-acting), incipient (slow-acting), or intermittent (non-continuous) faults. Early fall detection is a challenging task due to the masking effects of controllers (through their disturbance attenuation actions), the inverse relationship between lead time and false positive rates, and the temporal behavior of the faults/underlying factors. In this paper, we propose a fall detection algorithm that is capable of detecting both incipient and abrupt faults while maximizing lead time and meeting desired thresholds on the false positive and negative rates.

==> defines/PackageDefinitions.tex <==
% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}




\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{graphicx} 
\usepackage{grffile}
\usepackage[hypcap=true]{caption}
\usepackage{array}
\usepackage{mathtools}
\usepackage{commath}
\usepackage{colortbl}
\usepackage{enumerate}
\usepackage{hyperref}
\usepackage{cleveref}
% \usepackage{appendix}
\usepackage{subfig}
%\usepackage{subfloat}
\usepackage{float}
\usepackage{tabularx}
%\usepackage{subcaption}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{placeins}
\usepackage{hyperref}
\usepackage{tabu}

\usepackage{nomencl}
\makenomenclature

% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files


% \usepackage[compress]{cite}
%\usepackage{url}
%\usepackage{graphicx,xcolor}
%\usepackage{subcaption}
\usepackage{xfrac}
\usepackage{multicol}
%\usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}
\usepackage{soul}






\graphicspath{
    {template/}
}

\newcommand{\real}{\mathbb{R}} 

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


% \newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
% \newcommand{\mem}[1]{[{\textbf{\textcolor{blue}{MEM: #1}}}]}
% \newcommand{\mem}[1]{[{\textbf{\textcolor{blue}{MEM: #1}}}]}

\newcommand{\jwg}[1]{\textcolor{red}{{[\textbf{JWG: #1}]}}}
\newcommand{\mem}[1]{\textcolor{blue}{{[\textbf{MEM: #1}]}}}
\newcommand{\bh}[1]{\textcolor{note}{{[\textbf{Bruce: #1}]}}}
\definecolor{note}{rgb}{0.3,0.7,0.25}

\newcommand{\fnr}{\rm FNR}
\newcommand{\fpr}{\rm FPR}

\newcommand{\sts}{chair-to-stand}
\newcommand{\Sts}{Chair-to-stand}
\newcommand{\StS}{Chair-to-Stand}
\newcommand{\stc}{chair-to-crouch-to-stand}
\newcommand{\Stc}{Chair-to-crouch-to-stand}
\newcommand{\StC}{Chair-to-Crouch-to-Stand}


\newcounter{countitems}
\newcounter{nextitemizecount}
\newcommand{\setupcountitems}{%
  \stepcounter{nextitemizecount}%
  \setcounter{countitems}{0}%
  \preto\item{\stepcounter{countitems}}%
}
\makeatletter
\newcommand{\computecountitems}{%
  \edef\@currentlabel{\number\c@countitems}%
  \label{countitems@\number\numexpr\value{nextitemizecount}-1\relax}%
}
\newcommand{\nextitemizecount}{%
  \getrefnumber{countitems@\number\c@nextitemizecount}%
}
\newcommand{\previtemizecount}{%
  \getrefnumber{countitems@\number\numexpr\value{nextitemizecount}-1\relax}%
}
\makeatother    
\newenvironment{AutoMultiColItemize}{%
\ifnumcomp{\nextitemizecount}{>}{3}{\begin{multicols}{2}}{}%
\setupcountitems\begin{itemize}}%
{\end{itemize}%
\unskip\computecountitems\ifnumcomp{\previtemizecount}{>}{3}{\end{multicols}}{}}


\newcommand{\add}[1]{\textcolor{OliveGreen}{\textbf{#1}}}
\newcommand{\mdfy}[2]{\textcolor{Gray}{\st{#1}}\textcolor{Orange}{\textbf{#2}}}
\newcommand{\dels}[1]{\textcolor{Gray}{\st{\textbf{#1}}}}
\newcommand{\dlt}[1]{\textcolor{Gray}{#1}}

\DeclareRobustCommand{\hsout}[1]{\texorpdfstring{\st{#1}}{#1}} %https://tex.stackexchange.com/questions/22410/strikethrough-in-section-title

\usepackage[makeroom]{cancel}

\usepackage{stfloats}
\raggedbottom

==> img/fall_detection/classification_results/test.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
colorbar,
colorbar style={ytick={0.5,1,1.5,2,2.5,3},yticklabels={
  \(\displaystyle 0.5\),
  \(\displaystyle 1.0\),
  \(\displaystyle 1.5\),
  \(\displaystyle 2.0\),
  \(\displaystyle 2.5\),
  inf
},ylabel={Lead time}},
colormap/viridis,
point meta max=3,
point meta min=-0.348,
tick align=outside,
tick pos=left,
title={Nearest Neighbor Classification Incipient Fault},
x grid style={darkgray176},
xlabel={time (s)},
xmin=-0.221, xmax=5.961,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Decision function value},
ymin=-0.16155, ymax=3.39255,
ytick style={color=black}
]
\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.221, xmax=5.961,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1,
ytick style={color=black}
]
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.221, xmax=5.961,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1,
ytick style={color=black}
]
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.221, xmax=5.961,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1,
ytick style={color=black}
]
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.221, xmax=5.961,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1,
ytick style={color=black}
]
\end{axis}

\addplot [colormap/viridis, forget plot, only marks, scatter, scatter src=explicit]
table [x=x, y=y, meta=colordata]{%
x  y  colordata
0.06 0 3.0
0.09 0 3.0
0.12 0 3.0
0.15 0 3.0
0.17 0 3.0
0.2 0 3.0
0.23 0 3.0
0.26 0 3.0
0.29 0 3.0
0.32 0 3.0
0.35 0 3.0
0.38 0 3.0
0.41 0 3.0
0.44 0 3.0
0.46 0 3.0
0.49 0 3.0
0.52 0 3.0
0.55 0 3.0
0.58 0 3.0
0.61 0 3.0
0.64 0 3.0
0.67 0 3.0
0.7 0 3.0
0.72 0 3.0
0.75 0 3.0
0.78 0 3.0
0.81 0 3.0
0.84 0 3.0
0.87 0 3.0
0.9 0.001 3.0
0.93 0.001 3.0
0.96 0 3.0
0.99 0 3.0
1.01 0 3.0
1.04 0 3.0
1.07 0 3.0
1.1 0 3.0
1.13 0 3.0
1.16 0 3.0
1.19 0 3.0
1.22 0 3.0
1.25 0 3.0
1.28 0 3.0
1.3 0 3.0
1.33 0 3.0
1.36 0 3.0
1.39 0 3.0
1.42 0 3.0
1.45 0 3.0
1.48 0 3.0
1.51 0 3.0
1.54 0 3.0
1.57 0 3.0
1.59 0 3.0
1.62 0 3.0
1.65 0 3.0
1.68 0 3.0
1.71 0 3.0
1.74 0 3.0
1.77 0 3.0
1.8 0 3.0
1.83 0 3.0
1.86 0 3.0
1.88 0 3.0
1.91 0 3.0
1.94 0 3.0
1.97 0 3.0
2 0 3.0
2.03 0 3.0
2.06 0 3.0
2.09 0 3.0
2.12 0 3.0
2.15 0 3.0
2.17 0 3.0
2.2 0 3.0
2.23 0 3.0
2.26 0 3.0
2.29 0 3.0
2.32 0 3.0
2.35 0 3.0
2.38 0 3.0
2.41 0 3.0
2.44 0 3.0
2.46 0 3.0
2.49 0 3.0
2.52 0 3.0
2.55 0 3.0
2.58 0 3.0
2.61 0 3.0
2.64 0 3.0
2.67 0 3.0
2.7 0 3.0
2.73 0 3.0
2.76 0 3.0
2.78 0 3.0
2.81 0 3.0
2.84 0 3.0
2.87 0 3.0
2.9 0 3.0
2.93 0 3.0
2.96 0 3.0
2.99 0 3.0
3.02 0 3.0
3.04 0 3.0
3.07 0 3.0
3.1 0 3.0
3.13 0 3.0
3.16 0 3.0
3.19 0 3.0
3.22 0 3.0
3.25 0 3.0
3.28 0 3.0
3.31 0 3.0
3.34 0 3.0
3.36 0 3.0
3.39 0 3.0
3.42 0 3.0
3.45 0 3.0
3.48 0 3.0
3.51 0 3.0
3.54 0 3.0
3.57 0 3.0
3.6 0 3.0
3.62 0 3.0
3.65 0 3.0
3.68 0 3.0
3.71 0 3.0
3.74 0 3.0
3.77 0 3.0
3.8 0 3.0
3.83 0 3.0
3.86 0 3.0
3.89 0 3.0
3.92 0 3.0
3.94 0 3.0
3.97 0 3.0
4 0 3.0
4.03 0 3.0
4.06 0 3.0
4.09 0 3.0
4.12 0 3.0
4.15 0 3.0
4.18 0 3.0
4.2 0 3.0
4.23 0 3.0
4.26 0 3.0
4.29 0 3.0
4.32 0 3.0
4.35 0 3.0
4.38 0 3.0
4.41 0 3.0
4.44 0 3.0
4.47 0 3.0
4.5 0 3.0
4.52 0 3.0
4.55 0 3.0
4.58 0 3.0
4.61 0 3.0
4.64 0 3.0
4.67 0 3.0
4.7 0 3.0
4.73 0 3.0
4.76 0 3.0
4.78 0 3.0
4.81 0 3.0
4.84 0 3.0
4.87 0 3.0
4.9 0 3.0
4.93 0 3.0
4.96 0 3.0
4.99 0 3.0
5.02 0 3.0
5.05 0 3.0
5.08 0 3.0
5.1 0 3.0
5.13 0 3.0
5.16 0 3.0
5.19 0 3.0
5.22 0 3.0
5.25 0 3.0
5.28 0 3.0
5.31 0 3.0
5.34 0 3.0
5.36 0 3.0
5.39 0 3.0
5.42 0 3.0
5.45 0 3.0
5.48 0 3.0
5.51 0 3.0
5.54 0 3.0
5.57 0 3.0
5.6 0 3.0
5.63 0 3.0
5.66 0 3.0
5.68 0 3.0
0.06 0 3.0
0.09 0 3.0
0.12 0 3.0
0.15 0 3.0
0.17 0 3.0
0.2 0 3.0
0.23 0 3.0
0.26 0 3.0
0.29 0 3.0
0.32 0 3.0
0.35 0 3.0
0.38 0 3.0
0.41 0 3.0
0.44 0 3.0
0.46 0 3.0
0.49 0 3.0
0.52 0 3.0
0.55 0 3.0
0.58 0 3.0
0.61 0 3.0
0.64 0 3.0
0.67 0 3.0
0.7 0 3.0
0.73 0 3.0
0.75 0.001 3.0
0.78 0.001 3.0
0.81 0.001 3.0
0.84 0.001 3.0
0.87 0.001 3.0
0.9 0.002 3.0
0.93 0.002 3.0
0.96 0.002 3.0
0.99 0.002 3.0
1.02 0.001 3.0
1.04 0.001 3.0
1.07 0.001 3.0
1.1 0.001 3.0
1.13 0 3.0
1.16 0 3.0
1.19 0 3.0
1.22 0 3.0
1.25 0 3.0
1.28 0 3.0
1.31 0 3.0
1.33 0 3.0
1.36 0 3.0
1.39 0 3.0
1.42 0 3.0
1.45 0 3.0
1.48 0 3.0
1.51 0 3.0
1.54 0 3.0
1.57 0 3.0
1.59 0 3.0
1.62 0 3.0
1.65 0 3.0
1.68 0 3.0
1.71 0 3.0
1.74 0 3.0
1.77 0 3.0
1.8 0 3.0
1.83 0 3.0
1.86 0 3.0
1.88 0 3.0
1.91 0 3.0
1.94 0 3.0
1.97 0 3.0
2 0 3.0
2.03 0 3.0
2.06 0 3.0
2.09 0 3.0
2.12 0 3.0
2.15 0 3.0
2.17 0 3.0
2.2 0 3.0
2.23 0 3.0
2.26 0 3.0
2.29 0 3.0
2.32 0 3.0
2.35 0 3.0
2.38 0 3.0
2.41 0 3.0
2.44 0 3.0
2.46 0 3.0
2.49 0 3.0
2.52 0 3.0
2.55 0 3.0
2.58 0 3.0
2.61 0 3.0
2.64 0 3.0
2.67 0 3.0
2.7 0 3.0
2.73 0 3.0
2.76 0 3.0
2.78 0 3.0
2.81 0 3.0
2.84 0 3.0
2.87 0 3.0
2.9 0 3.0
2.93 0 3.0
2.96 0 3.0
2.99 0 3.0
3.02 0 3.0
3.04 0 3.0
3.07 0 3.0
3.1 0 3.0
3.13 0 3.0
3.16 0 3.0
3.19 0 3.0
3.22 0 3.0
3.25 0 3.0
3.28 0 3.0
3.31 0 3.0
3.33 0 3.0
3.36 0 3.0
3.39 0 3.0
3.42 0 3.0
3.45 0 3.0
3.48 0 3.0
3.51 0 3.0
3.54 0 3.0
3.57 0 3.0
3.6 0 3.0
3.62 0 3.0
3.65 0 3.0
3.68 0 3.0
3.71 0 3.0
3.74 0 3.0
3.77 0 3.0
3.8 0 3.0
3.83 0 3.0
3.86 0 3.0
3.89 0 3.0
3.91 0 3.0
3.94 0 3.0
3.97 0 3.0
4 0 3.0
4.03 0 3.0
4.06 0 3.0
4.09 0 3.0
4.12 0 3.0
4.15 0 3.0
4.18 0 3.0
4.2 0 3.0
4.23 0 3.0
4.26 0 3.0
4.29 0 3.0
4.32 0 3.0
4.35 0 3.0
4.38 0 3.0
4.41 0 3.0
4.44 0 3.0
4.47 0 3.0
4.49 0 3.0
4.52 0 3.0
4.55 0 3.0
4.58 0 3.0
4.61 0 3.0
4.64 0 3.0
4.67 0 3.0
4.7 0 3.0
4.73 0 3.0
4.76 0 3.0
4.78 0 3.0
4.81 0 3.0
4.84 0 3.0
4.87 0 3.0
4.9 0 3.0
4.93 0 3.0
4.96 0 3.0
4.99 0 3.0
5.02 0 3.0
5.05 0 3.0
5.08 0 3.0
5.1 0 3.0
5.13 0 3.0
5.16 0 3.0
5.19 0 3.0
5.22 0 3.0
5.25 0 3.0
5.28 0 3.0
5.31 0 3.0
5.34 0 3.0
5.36 0 3.0
5.39 0 3.0
5.42 0 3.0
5.45 0 3.0
5.48 0 3.0
5.51 0 3.0
5.54 0 3.0
5.57 0 3.0
5.6 0 3.0
5.63 0 3.0
5.65 0 3.0
5.68 0 3.0
0.06 0.001 3.0
0.09 0 3.0
0.12 0 3.0
0.15 0 3.0
0.17 0 3.0
0.2 0 3.0
0.23 0 3.0
0.26 0 3.0
0.29 0 3.0
0.32 0 3.0
0.35 0 3.0
0.38 0 3.0
0.41 0 3.0
0.44 0 3.0
0.46 0 3.0
0.49 0 3.0
0.52 0 3.0
0.55 0 3.0
0.58 0.001 3.0
0.61 0.001 3.0
0.64 0.001 3.0
0.67 0.001 3.0
0.7 0.001 3.0
0.73 0.001 3.0
0.75 0.002 3.0
0.78 0.002 3.0
0.81 0.001 3.0
0.84 0.001 3.0
0.87 0.001 3.0
0.9 0.001 3.0
0.93 0.002 3.0
0.96 0.002 3.0
0.99 0.002 3.0
1.02 0.002 3.0
1.04 0.002 3.0
1.07 0.002 3.0
1.1 0.002 3.0
1.13 0.002 3.0
1.16 0.001 3.0
1.19 0.001 3.0
1.22 0.001 3.0
1.25 0.001 3.0
1.28 0.001 3.0
1.31 0.001 3.0
1.33 0 3.0
1.36 0 3.0
1.39 0 3.0
1.42 0 3.0
1.45 0 3.0
1.48 0 3.0
1.51 0 3.0
1.54 0 3.0
1.57 0 3.0
1.6 0 3.0
1.62 0 3.0
1.65 0 3.0
1.68 0 3.0
1.71 0 3.0
1.74 0 3.0
1.77 0 3.0
1.8 0 3.0
1.83 0 3.0
1.86 0 3.0
1.89 0 3.0
1.91 0 3.0
1.94 0 3.0
1.97 0 3.0
2 0 3.0
2.03 0 3.0
2.06 0 3.0
2.09 0 3.0
2.12 0 3.0
2.15 0 3.0
2.17 0 3.0
2.2 0 3.0
2.23 0 3.0
2.26 0 3.0
2.29 0 3.0
2.32 0 3.0
2.35 0 3.0
2.38 0 3.0
2.41 0 3.0
2.44 0 3.0
2.46 0 3.0
2.49 0 3.0
2.52 0 3.0
2.55 0 3.0
2.58 0 3.0
2.61 0 3.0
2.64 0 3.0
2.67 0 3.0
2.7 0 3.0
2.73 0 3.0
2.75 0 3.0
2.78 0 3.0
2.81 0 3.0
2.84 0 3.0
2.87 0 3.0
2.9 0 3.0
2.93 0 3.0
2.96 0 3.0
2.99 0 3.0
3.02 0 3.0
3.05 0 3.0
3.07 0 3.0
3.1 0 3.0
3.13 0 3.0
3.16 0 3.0
3.19 0 3.0
3.22 0 3.0
3.25 0 3.0
3.28 0 3.0
3.31 0 3.0
3.33 0 3.0
3.36 0 3.0
3.39 0 3.0
3.42 0 3.0
3.45 0 3.0
3.48 0 3.0
3.51 0 3.0
3.54 0 3.0
3.57 0 3.0
3.6 0 3.0
3.63 0 3.0
3.65 0 3.0
3.68 0 3.0
3.71 0 3.0
3.74 0 3.0
3.77 0 3.0
3.8 0 3.0
3.83 0 3.0
3.86 0 3.0
3.89 0 3.0
3.91 0 3.0
3.94 0 3.0
3.97 0 3.0
4 0 3.0
4.03 0 3.0
4.06 0 3.0
4.09 0 3.0
4.12 0 3.0
4.15 0 3.0
4.18 0 3.0
4.2 0 3.0
4.23 0 3.0
4.26 0 3.0
4.29 0 3.0
4.32 0 3.0
4.35 0 3.0
4.38 0 3.0
4.41 0 3.0
4.44 0 3.0
4.47 0 3.0
4.49 0 3.0
4.52 0 3.0
4.55 0 3.0
4.58 0 3.0
4.61 0 3.0
4.64 0 3.0
4.67 0 3.0
4.7 0 3.0
4.73 0 3.0
4.76 0 3.0
4.78 0 3.0
4.81 0 3.0
4.84 0 3.0
4.87 0 3.0
4.9 0 3.0
4.93 0 3.0
4.96 0 3.0
4.99 0 3.0
5.02 0 3.0
5.05 0 3.0
5.07 0 3.0
5.1 0 3.0
5.13 0 3.0
5.16 0 3.0
5.19 0 3.0
5.22 0 3.0
5.25 0 3.0
5.28 0 3.0
5.31 0 3.0
5.34 0 3.0
5.36 0 3.0
5.39 0 3.0
5.42 0 3.0
5.45 0 3.0
5.48 0 3.0
5.51 0 3.0
5.54 0 3.0
5.57 0 3.0
5.6 0 3.0
5.63 0 3.0
5.65 0 3.0
5.68 0 3.0
0.06 0.001 1.392
0.09 0.001 1.363
0.12 0.001 1.3339999999999996
0.15 0.001 1.3049999999999997
0.17 0.001 1.2759999999999998
0.2 0.001 1.2469999999999999
0.23 0.001 1.218
0.26 0.001 1.1889999999999996
0.29 0.001 1.1599999999999997
0.32 0.002 1.1309999999999998
0.35 0.002 1.1019999999999999
0.38 0.002 1.073
0.41 0.003 1.044
0.44 0.004 1.0149999999999997
0.46 0.005 0.9859999999999998
0.49 0.006 0.9569999999999999
0.52 0.007 0.9279999999999999
0.55 0.008 0.899
0.58 0.01 0.8699999999999997
0.61 0.013 0.8409999999999997
0.64 0.016 0.8119999999999998
0.67 0.019 0.7829999999999999
0.7 0.023 0.754
0.73 0.028 0.7249999999999996
0.75 0.034 0.6959999999999997
0.78 0.039 0.6669999999999998
0.81 0.04 0.6379999999999999
0.84 0.039 0.609
0.87 0.037 0.5799999999999996
0.9 0.037 0.5509999999999997
0.93 0.042 0.5219999999999998
0.96 0.055 0.4929999999999999
0.99 0.073 0.46399999999999997
1.02 0.089 0.4349999999999996
1.04 0.093 0.4059999999999997
1.07 0.089 0.3769999999999998
1.1 0.094 0.34799999999999986
1.13 0.14 0.31899999999999995
1.16 0.287 0.2899999999999996
1.19 0.455 0.2609999999999997
1.22 0.46 0.2320000000000002
1.25 0.396 0.2029999999999994
1.28 0.361 0.1739999999999995
1.31 0.326 0.14499999999999957
1.33 0.25 0.11599999999999966
1.36 0.192 0.08699999999999974
1.39 0.199 0.05799999999999983
1.42 0.228 0.028999999999999915
1.45 0.404 0.0
1.48 1.945 -0.028999999999999915
1.51 2.588 -0.05799999999999983
1.54 1.384 -0.08700000000000063
1.57 0.848 -0.11600000000000055
1.6 1.024 -0.14500000000000046
1.62 1.401 -0.17400000000000038
1.65 1.673 -0.2030000000000003
1.68 1.928 -0.2320000000000002
1.71 2.102 -0.2610000000000001
1.74 2.252 -0.29000000000000004
1.77 2.564 -0.31899999999999995
1.8 2.893 -0.34799999999999986
0.06 0.002 1.4500000000000002
0.09 0.002 1.4210000000000003
0.12 0.003 1.3920000000000003
0.15 0.003 1.3630000000000004
0.17 0.004 1.334
0.2 0.005 1.3050000000000002
0.23 0.006 1.2760000000000002
0.26 0.007 1.2470000000000003
0.29 0.009 1.2180000000000004
0.32 0.012 1.189
0.35 0.014 1.1600000000000001
0.38 0.017 1.1310000000000002
0.41 0.021 1.1020000000000003
0.44 0.025 1.0730000000000004
0.46 0.031 1.044
0.49 0.038 1.0150000000000001
0.52 0.046 0.9860000000000002
0.55 0.057 0.9570000000000003
0.58 0.068 0.9280000000000004
0.61 0.082 0.899
0.64 0.099 0.8700000000000001
0.67 0.119 0.8410000000000002
0.7 0.145 0.8120000000000003
0.73 0.176 0.7830000000000004
0.75 0.209 0.754
0.78 0.233 0.7250000000000001
0.81 0.237 0.6960000000000002
0.84 0.229 0.6670000000000003
0.87 0.239 0.6380000000000003
0.9 0.342 0.6090000000000004
0.93 0.773 0.5800000000000001
0.96 1.171 0.5510000000000002
0.99 1.068 0.5220000000000002
1.02 0.734 0.4930000000000003
1.04 0.443 0.4640000000000004
1.07 0.312 0.43500000000000005
1.1 0.313 0.40600000000000014
1.13 0.37 0.3770000000000002
1.16 0.394 0.3480000000000003
1.19 0.514 0.3190000000000004
1.22 0.975 0.29000000000000004
1.25 1.152 0.2610000000000001
1.28 1.271 0.2320000000000002
1.31 1.775 0.2030000000000003
1.33 2.223 0.17400000000000038
1.36 2.522 0.14500000000000002
1.39 2.627 0.1160000000000001
1.42 2.875 0.08700000000000019
1.45 3.231 0.058000000000000274
0.06 0.005 1.1600000000000001
0.09 0.006 1.1310000000000002
0.12 0.008 1.1020000000000003
0.15 0.009 1.0730000000000004
0.17 0.011 1.044
0.2 0.013 1.0150000000000001
0.23 0.017 0.9860000000000002
0.26 0.021 0.9570000000000003
0.29 0.026 0.9280000000000004
0.32 0.031 0.899
0.35 0.037 0.8700000000000001
0.38 0.045 0.8410000000000002
0.41 0.055 0.8120000000000003
0.44 0.067 0.7830000000000004
0.46 0.083 0.754
0.49 0.101 0.7250000000000001
0.52 0.121 0.6960000000000002
0.55 0.143 0.6670000000000003
0.58 0.169 0.6380000000000003
0.61 0.203 0.609
0.64 0.248 0.5800000000000001
0.67 0.3 0.5510000000000002
0.7 0.345 0.5220000000000002
0.73 0.365 0.4930000000000003
0.75 0.372 0.4640000000000004
0.78 0.432 0.43500000000000005
0.81 0.764 0.40600000000000014
0.84 1.292 0.3770000000000002
0.87 1.244 0.3480000000000003
0.9 0.724 0.3190000000000004
0.93 0.53 0.29000000000000004
0.96 0.524 0.2610000000000001
0.99 0.464 0.2320000000000002
1.02 0.524 0.2030000000000003
1.04 0.643 0.17400000000000038
1.07 0.685 0.14500000000000002
1.1 1.878 0.1160000000000001
1.13 2.24 0.08700000000000019
1.16 1.395 0.058000000000000274
1.19 2.24 0.02900000000000036
1.22 3.106 0.0
1.25 3.138 -0.028999999999999915
};
\addplot [semithick, steelblue31119180, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0
0.09 0
0.12 0
0.15 0
0.17 0
0.2 0
0.23 0
0.26 0
0.29 0
0.32 0
0.35 0
0.38 0
0.41 0
0.44 0
0.46 0
0.49 0
0.52 0
0.55 0
0.58 0
0.61 0
0.64 0
0.67 0
0.7 0
0.72 0
0.75 0
0.78 0
0.81 0
0.84 0
0.87 0
0.9 0.001
0.93 0.001
0.96 0
0.99 0
1.01 0
1.04 0
1.07 0
1.1 0
1.13 0
1.16 0
1.19 0
1.22 0
1.25 0
1.28 0
1.3 0
1.33 0
1.36 0
1.39 0
1.42 0
1.45 0
1.48 0
1.51 0
1.54 0
1.57 0
1.59 0
1.62 0
1.65 0
1.68 0
1.71 0
1.74 0
1.77 0
1.8 0
1.83 0
1.86 0
1.88 0
1.91 0
1.94 0
1.97 0
2 0
2.03 0
2.06 0
2.09 0
2.12 0
2.15 0
2.17 0
2.2 0
2.23 0
2.26 0
2.29 0
2.32 0
2.35 0
2.38 0
2.41 0
2.44 0
2.46 0
2.49 0
2.52 0
2.55 0
2.58 0
2.61 0
2.64 0
2.67 0
2.7 0
2.73 0
2.76 0
2.78 0
2.81 0
2.84 0
2.87 0
2.9 0
2.93 0
2.96 0
2.99 0
3.02 0
3.04 0
3.07 0
3.1 0
3.13 0
3.16 0
3.19 0
3.22 0
3.25 0
3.28 0
3.31 0
3.34 0
3.36 0
3.39 0
3.42 0
3.45 0
3.48 0
3.51 0
3.54 0
3.57 0
3.6 0
3.62 0
3.65 0
3.68 0
3.71 0
3.74 0
3.77 0
3.8 0
3.83 0
3.86 0
3.89 0
3.92 0
3.94 0
3.97 0
4 0
4.03 0
4.06 0
4.09 0
4.12 0
4.15 0
4.18 0
4.2 0
4.23 0
4.26 0
4.29 0
4.32 0
4.35 0
4.38 0
4.41 0
4.44 0
4.47 0
4.5 0
4.52 0
4.55 0
4.58 0
4.61 0
4.64 0
4.67 0
4.7 0
4.73 0
4.76 0
4.78 0
4.81 0
4.84 0
4.87 0
4.9 0
4.93 0
4.96 0
4.99 0
5.02 0
5.05 0
5.08 0
5.1 0
5.13 0
5.16 0
5.19 0
5.22 0
5.25 0
5.28 0
5.31 0
5.34 0
5.36 0
5.39 0
5.42 0
5.45 0
5.48 0
5.51 0
5.54 0
5.57 0
5.6 0
5.63 0
5.66 0
5.68 0
};
\addlegendentry{14.3 N}
\addplot [semithick, darkorange25512714, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0
0.09 0
0.12 0
0.15 0
0.17 0
0.2 0
0.23 0
0.26 0
0.29 0
0.32 0
0.35 0
0.38 0
0.41 0
0.44 0
0.46 0
0.49 0
0.52 0
0.55 0
0.58 0
0.61 0
0.64 0
0.67 0
0.7 0
0.73 0
0.75 0.001
0.78 0.001
0.81 0.001
0.84 0.001
0.87 0.001
0.9 0.002
0.93 0.002
0.96 0.002
0.99 0.002
1.02 0.001
1.04 0.001
1.07 0.001
1.1 0.001
1.13 0
1.16 0
1.19 0
1.22 0
1.25 0
1.28 0
1.31 0
1.33 0
1.36 0
1.39 0
1.42 0
1.45 0
1.48 0
1.51 0
1.54 0
1.57 0
1.59 0
1.62 0
1.65 0
1.68 0
1.71 0
1.74 0
1.77 0
1.8 0
1.83 0
1.86 0
1.88 0
1.91 0
1.94 0
1.97 0
2 0
2.03 0
2.06 0
2.09 0
2.12 0
2.15 0
2.17 0
2.2 0
2.23 0
2.26 0
2.29 0
2.32 0
2.35 0
2.38 0
2.41 0
2.44 0
2.46 0
2.49 0
2.52 0
2.55 0
2.58 0
2.61 0
2.64 0
2.67 0
2.7 0
2.73 0
2.76 0
2.78 0
2.81 0
2.84 0
2.87 0
2.9 0
2.93 0
2.96 0
2.99 0
3.02 0
3.04 0
3.07 0
3.1 0
3.13 0
3.16 0
3.19 0
3.22 0
3.25 0
3.28 0
3.31 0
3.33 0
3.36 0
3.39 0
3.42 0
3.45 0
3.48 0
3.51 0
3.54 0
3.57 0
3.6 0
3.62 0
3.65 0
3.68 0
3.71 0
3.74 0
3.77 0
3.8 0
3.83 0
3.86 0
3.89 0
3.91 0
3.94 0
3.97 0
4 0
4.03 0
4.06 0
4.09 0
4.12 0
4.15 0
4.18 0
4.2 0
4.23 0
4.26 0
4.29 0
4.32 0
4.35 0
4.38 0
4.41 0
4.44 0
4.47 0
4.49 0
4.52 0
4.55 0
4.58 0
4.61 0
4.64 0
4.67 0
4.7 0
4.73 0
4.76 0
4.78 0
4.81 0
4.84 0
4.87 0
4.9 0
4.93 0
4.96 0
4.99 0
5.02 0
5.05 0
5.08 0
5.1 0
5.13 0
5.16 0
5.19 0
5.22 0
5.25 0
5.28 0
5.31 0
5.34 0
5.36 0
5.39 0
5.42 0
5.45 0
5.48 0
5.51 0
5.54 0
5.57 0
5.6 0
5.63 0
5.65 0
5.68 0
};
\addlegendentry{21.39 N}
\addplot [semithick, forestgreen4416044, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0.001
0.09 0
0.12 0
0.15 0
0.17 0
0.2 0
0.23 0
0.26 0
0.29 0
0.32 0
0.35 0
0.38 0
0.41 0
0.44 0
0.46 0
0.49 0
0.52 0
0.55 0
0.58 0.001
0.61 0.001
0.64 0.001
0.67 0.001
0.7 0.001
0.73 0.001
0.75 0.002
0.78 0.002
0.81 0.001
0.84 0.001
0.87 0.001
0.9 0.001
0.93 0.002
0.96 0.002
0.99 0.002
1.02 0.002
1.04 0.002
1.07 0.002
1.1 0.002
1.13 0.002
1.16 0.001
1.19 0.001
1.22 0.001
1.25 0.001
1.28 0.001
1.31 0.001
1.33 0
1.36 0
1.39 0
1.42 0
1.45 0
1.48 0
1.51 0
1.54 0
1.57 0
1.6 0
1.62 0
1.65 0
1.68 0
1.71 0
1.74 0
1.77 0
1.8 0
1.83 0
1.86 0
1.89 0
1.91 0
1.94 0
1.97 0
2 0
2.03 0
2.06 0
2.09 0
2.12 0
2.15 0
2.17 0
2.2 0
2.23 0
2.26 0
2.29 0
2.32 0
2.35 0
2.38 0
2.41 0
2.44 0
2.46 0
2.49 0
2.52 0
2.55 0
2.58 0
2.61 0
2.64 0
2.67 0
2.7 0
2.73 0
2.75 0
2.78 0
2.81 0
2.84 0
2.87 0
2.9 0
2.93 0
2.96 0
2.99 0
3.02 0
3.05 0
3.07 0
3.1 0
3.13 0
3.16 0
3.19 0
3.22 0
3.25 0
3.28 0
3.31 0
3.33 0
3.36 0
3.39 0
3.42 0
3.45 0
3.48 0
3.51 0
3.54 0
3.57 0
3.6 0
3.63 0
3.65 0
3.68 0
3.71 0
3.74 0
3.77 0
3.8 0
3.83 0
3.86 0
3.89 0
3.91 0
3.94 0
3.97 0
4 0
4.03 0
4.06 0
4.09 0
4.12 0
4.15 0
4.18 0
4.2 0
4.23 0
4.26 0
4.29 0
4.32 0
4.35 0
4.38 0
4.41 0
4.44 0
4.47 0
4.49 0
4.52 0
4.55 0
4.58 0
4.61 0
4.64 0
4.67 0
4.7 0
4.73 0
4.76 0
4.78 0
4.81 0
4.84 0
4.87 0
4.9 0
4.93 0
4.96 0
4.99 0
5.02 0
5.05 0
5.07 0
5.1 0
5.13 0
5.16 0
5.19 0
5.22 0
5.25 0
5.28 0
5.31 0
5.34 0
5.36 0
5.39 0
5.42 0
5.45 0
5.48 0
5.51 0
5.54 0
5.57 0
5.6 0
5.63 0
5.65 0
5.68 0
};
\addlegendentry{22.5 N}
\addplot [semithick, crimson2143940, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0.001
0.09 0.001
0.12 0.001
0.15 0.001
0.17 0.001
0.2 0.001
0.23 0.001
0.26 0.001
0.29 0.001
0.32 0.002
0.35 0.002
0.38 0.002
0.41 0.003
0.44 0.004
0.46 0.005
0.49 0.006
0.52 0.007
0.55 0.008
0.58 0.01
0.61 0.013
0.64 0.016
0.67 0.019
0.7 0.023
0.73 0.028
0.75 0.034
0.78 0.039
0.81 0.04
0.84 0.039
0.87 0.037
0.9 0.037
0.93 0.042
0.96 0.055
0.99 0.073
1.02 0.089
1.04 0.093
1.07 0.089
1.1 0.094
1.13 0.14
1.16 0.287
1.19 0.455
1.22 0.46
1.25 0.396
1.28 0.361
1.31 0.326
1.33 0.25
1.36 0.192
1.39 0.199
1.42 0.228
1.45 0.404
1.48 1.945
1.51 2.588
1.54 1.384
1.57 0.848
1.6 1.024
1.62 1.401
1.65 1.673
1.68 1.928
1.71 2.102
1.74 2.252
1.77 2.564
1.8 2.893
};
\addlegendentry{28.53 N}
\addplot [semithick, mediumpurple148103189, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0.002
0.09 0.002
0.12 0.003
0.15 0.003
0.17 0.004
0.2 0.005
0.23 0.006
0.26 0.007
0.29 0.009
0.32 0.012
0.35 0.014
0.38 0.017
0.41 0.021
0.44 0.025
0.46 0.031
0.49 0.038
0.52 0.046
0.55 0.057
0.58 0.068
0.61 0.082
0.64 0.099
0.67 0.119
0.7 0.145
0.73 0.176
0.75 0.209
0.78 0.233
0.81 0.237
0.84 0.229
0.87 0.239
0.9 0.342
0.93 0.773
0.96 1.171
0.99 1.068
1.02 0.734
1.04 0.443
1.07 0.312
1.1 0.313
1.13 0.37
1.16 0.394
1.19 0.514
1.22 0.975
1.25 1.152
1.28 1.271
1.31 1.775
1.33 2.223
1.36 2.522
1.39 2.627
1.42 2.875
1.45 3.231
};
\addlegendentry{36.02 N}
\addplot [semithick, sienna1408675, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0.005
0.09 0.006
0.12 0.008
0.15 0.009
0.17 0.011
0.2 0.013
0.23 0.017
0.26 0.021
0.29 0.026
0.32 0.031
0.35 0.037
0.38 0.045
0.41 0.055
0.44 0.067
0.46 0.083
0.49 0.101
0.52 0.121
0.55 0.143
0.58 0.169
0.61 0.203
0.64 0.248
0.67 0.3
0.7 0.345
0.73 0.365
0.75 0.372
0.78 0.432
0.81 0.764
0.84 1.292
0.87 1.244
0.9 0.724
0.93 0.53
0.96 0.524
0.99 0.464
1.02 0.524
1.04 0.643
1.07 0.685
1.1 1.878
1.13 2.24
1.16 1.395
1.19 2.24
1.22 3.106
1.25 3.138
};
\addlegendentry{41.26 N}
\addplot [semithick, red, forget plot]
table {%
-0.221 0.003
5.961 0.003
};
\end{axis}

\end{tikzpicture}


==> img/fall_detection/classification_results/test_old.tex <==
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
colorbar,
colorbar style={ytick={0.5,1,1.5,2,2.5,3},yticklabels={
  \(\displaystyle 0.5\),
  \(\displaystyle 1.0\),
  \(\displaystyle 1.5\),
  \(\displaystyle 2.0\),
  \(\displaystyle 2.5\),
  inf
},ylabel={Lead time}},
colormap/viridis,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
point meta max=3,
point meta min=-0.0290000000000008,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time (s)},
xmin=-0.221, xmax=5.961,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Classification decision function},
ymin=-0.16335, ymax=3.43035,
ytick style={color=black}
]
\addplot [colormap/viridis, forget plot, only marks, scatter, scatter src=explicit]
table [x=x, y=y, meta=colordata]{%
x  y  colordata
0.06 0.003 1.2179999999999995
0.09 0.004 1.1889999999999996
0.12 0.005 1.1599999999999997
0.15 0.006 1.1309999999999998
0.17 0.007 1.1019999999999994
0.2 0.009 1.0729999999999995
0.23 0.011 1.0439999999999996
0.26 0.013 1.0149999999999997
0.29 0.017 0.9859999999999998
0.32 0.021 0.9569999999999994
0.35 0.025 0.9279999999999995
0.38 0.03 0.8989999999999996
0.41 0.036 0.8699999999999997
0.44 0.044 0.8409999999999997
0.46 0.054 0.8119999999999994
0.49 0.067 0.7829999999999995
0.52 0.081 0.7539999999999996
0.55 0.097 0.7249999999999996
0.58 0.116 0.6959999999999997
0.61 0.138 0.6669999999999994
0.64 0.167 0.6379999999999995
0.67 0.204 0.609
0.7 0.245 0.5799999999999992
0.73 0.285 0.5509999999999993
0.75 0.316 0.5219999999999994
0.78 0.332 0.49299999999999944
0.81 0.345 0.4639999999999995
0.84 0.407 0.4349999999999996
0.87 0.659 0.4059999999999997
0.9 0.992 0.3769999999999998
0.93 0.862 0.34799999999999986
0.96 0.573 0.31899999999999995
0.99 0.454 0.28999999999999915
1.02 0.422 0.26099999999999923
1.04 0.48 0.23199999999999932
1.07 0.526 0.2029999999999994
1.1 1.906 0.1739999999999995
1.13 2.133 0.14499999999999957
1.16 1.116 0.11599999999999966
1.19 1.619 0.08699999999999974
1.22 2.102 0.05799999999999983
1.25 2.152 0.028999999999999915
1.28 2.172 0.0
1.31 2.271 -0.029000000000000803
0.06 0 3.0
0.09 0 3.0
0.12 0 3.0
0.14 0 3.0
0.17 0 3.0
0.2 0 3.0
0.23 0 3.0
0.26 0 3.0
0.29 0 3.0
0.32 0 3.0
0.35 0 3.0
0.38 0 3.0
0.41 0 3.0
0.43 0 3.0
0.46 0 3.0
0.49 0 3.0
0.52 0 3.0
0.55 0 3.0
0.58 0 3.0
0.61 0 3.0
0.64 0 3.0
0.67 0 3.0
0.7 0 3.0
0.72 0 3.0
0.75 0 3.0
0.78 0 3.0
0.81 0 3.0
0.84 0 3.0
0.87 0 3.0
0.9 0 3.0
0.93 0 3.0
0.96 0 3.0
0.99 0 3.0
1.01 0 3.0
1.04 0 3.0
1.07 0 3.0
1.1 0 3.0
1.13 0 3.0
1.16 0 3.0
1.19 0 3.0
1.22 0 3.0
1.25 0 3.0
1.28 0 3.0
1.3 0 3.0
1.33 0 3.0
1.36 0 3.0
1.39 0 3.0
1.42 0 3.0
1.45 0 3.0
1.48 0 3.0
1.51 0 3.0
1.54 0 3.0
1.57 0 3.0
1.59 0 3.0
1.62 0 3.0
1.65 0 3.0
1.68 0 3.0
1.71 0 3.0
1.74 0 3.0
1.77 0 3.0
1.8 0 3.0
1.83 0 3.0
1.86 0 3.0
1.88 0 3.0
1.91 0 3.0
1.94 0 3.0
1.97 0 3.0
2 0 3.0
2.03 0 3.0
2.06 0 3.0
2.09 0 3.0
2.12 0 3.0
2.15 0 3.0
2.17 0 3.0
2.2 0 3.0
2.23 0 3.0
2.26 0 3.0
2.29 0 3.0
2.32 0 3.0
2.35 0 3.0
2.38 0 3.0
2.41 0 3.0
2.44 0 3.0
2.46 0 3.0
2.49 0 3.0
2.52 0 3.0
2.55 0 3.0
2.58 0 3.0
2.61 0 3.0
2.64 0 3.0
2.67 0 3.0
2.7 0 3.0
2.73 0 3.0
2.76 0 3.0
2.78 0 3.0
2.81 0 3.0
2.84 0 3.0
2.87 0 3.0
2.9 0 3.0
2.93 0 3.0
2.96 0 3.0
2.99 0 3.0
3.02 0 3.0
3.04 0 3.0
3.07 0 3.0
3.1 0 3.0
3.13 0 3.0
3.16 0 3.0
3.19 0 3.0
3.22 0 3.0
3.25 0 3.0
3.28 0 3.0
3.31 0 3.0
3.34 0 3.0
3.36 0 3.0
3.39 0 3.0
3.42 0 3.0
3.45 0 3.0
3.48 0 3.0
3.51 0 3.0
3.54 0 3.0
3.57 0 3.0
3.6 0 3.0
3.62 0 3.0
3.65 0 3.0
3.68 0 3.0
3.71 0 3.0
3.74 0 3.0
3.77 0 3.0
3.8 0 3.0
3.83 0 3.0
3.86 0 3.0
3.89 0 3.0
3.92 0 3.0
3.94 0 3.0
3.97 0 3.0
4 0 3.0
4.03 0 3.0
4.06 0 3.0
4.09 0 3.0
4.12 0 3.0
4.15 0 3.0
4.18 0 3.0
4.2 0 3.0
4.23 0 3.0
4.26 0 3.0
4.29 0 3.0
4.32 0 3.0
4.35 0 3.0
4.38 0 3.0
4.41 0 3.0
4.44 0 3.0
4.47 0 3.0
4.5 0 3.0
4.52 0 3.0
4.55 0 3.0
4.58 0 3.0
4.61 0 3.0
4.64 0 3.0
4.67 0 3.0
4.7 0 3.0
4.73 0 3.0
4.76 0 3.0
4.78 0 3.0
4.81 0 3.0
4.84 0 3.0
4.87 0 3.0
4.9 0 3.0
4.93 0 3.0
4.96 0 3.0
4.99 0 3.0
5.02 0 3.0
5.05 0 3.0
5.08 0 3.0
5.1 0 3.0
5.13 0 3.0
5.16 0 3.0
5.19 0 3.0
5.22 0 3.0
5.25 0 3.0
5.28 0 3.0
5.31 0 3.0
5.34 0 3.0
5.36 0 3.0
5.39 0 3.0
5.42 0 3.0
5.45 0 3.0
5.48 0 3.0
5.51 0 3.0
5.54 0 3.0
5.57 0 3.0
5.6 0 3.0
5.63 0 3.0
5.66 0 3.0
5.68 0 3.0
0.06 0 3.0
0.09 0 3.0
0.12 0 3.0
0.15 0 3.0
0.17 0 3.0
0.2 0 3.0
0.23 0 3.0
0.26 0 3.0
0.29 0 3.0
0.32 0 3.0
0.35 0 3.0
0.38 0 3.0
0.41 0 3.0
0.44 0 3.0
0.46 0 3.0
0.49 0 3.0
0.52 0 3.0
0.55 0 3.0
0.58 0 3.0
0.61 0 3.0
0.64 0 3.0
0.67 0 3.0
0.7 0 3.0
0.73 0 3.0
0.75 0 3.0
0.78 0 3.0
0.81 0 3.0
0.84 0 3.0
0.87 0 3.0
0.9 0 3.0
0.93 0 3.0
0.96 0 3.0
0.99 0 3.0
1.01 0 3.0
1.04 0 3.0
1.07 0 3.0
1.1 0 3.0
1.13 0 3.0
1.16 0 3.0
1.19 0 3.0
1.22 0 3.0
1.25 0 3.0
1.28 0 3.0
1.3 0 3.0
1.33 0 3.0
1.36 0 3.0
1.39 0 3.0
1.42 0 3.0
1.45 0 3.0
1.48 0 3.0
1.51 0 3.0
1.54 0 3.0
1.57 0 3.0
1.59 0 3.0
1.62 0 3.0
1.65 0 3.0
1.68 0 3.0
1.71 0 3.0
1.74 0 3.0
1.77 0 3.0
1.8 0 3.0
1.83 0 3.0
1.86 0 3.0
1.88 0 3.0
1.91 0 3.0
1.94 0 3.0
1.97 0 3.0
2 0 3.0
2.03 0 3.0
2.06 0 3.0
2.09 0 3.0
2.12 0 3.0
2.15 0 3.0
2.17 0 3.0
2.2 0 3.0
2.23 0 3.0
2.26 0 3.0
2.29 0 3.0
2.32 0 3.0
2.35 0 3.0
2.38 0 3.0
2.41 0 3.0
2.44 0 3.0
2.46 0 3.0
2.49 0 3.0
2.52 0 3.0
2.55 0 3.0
2.58 0 3.0
2.61 0 3.0
2.64 0 3.0
2.67 0 3.0
2.7 0 3.0
2.73 0 3.0
2.76 0 3.0
2.78 0 3.0
2.81 0 3.0
2.84 0 3.0
2.87 0 3.0
2.9 0 3.0
2.93 0 3.0
2.96 0 3.0
2.99 0 3.0
3.02 0 3.0
3.04 0 3.0
3.07 0 3.0
3.1 0 3.0
3.13 0 3.0
3.16 0 3.0
3.19 0 3.0
3.22 0 3.0
3.25 0 3.0
3.28 0 3.0
3.31 0 3.0
3.34 0 3.0
3.36 0 3.0
3.39 0 3.0
3.42 0 3.0
3.45 0 3.0
3.48 0 3.0
3.51 0 3.0
3.54 0 3.0
3.57 0 3.0
3.6 0 3.0
3.62 0 3.0
3.65 0 3.0
3.68 0 3.0
3.71 0 3.0
3.74 0 3.0
3.77 0 3.0
3.8 0 3.0
3.83 0 3.0
3.86 0 3.0
3.89 0 3.0
3.92 0 3.0
3.94 0 3.0
3.97 0 3.0
4 0 3.0
4.03 0 3.0
4.06 0 3.0
4.09 0 3.0
4.12 0 3.0
4.15 0 3.0
4.18 0 3.0
4.2 0 3.0
4.23 0 3.0
4.26 0 3.0
4.29 0 3.0
4.32 0 3.0
4.35 0 3.0
4.38 0 3.0
4.41 0 3.0
4.44 0 3.0
4.47 0 3.0
4.5 0 3.0
4.52 0 3.0
4.55 0 3.0
4.58 0 3.0
4.61 0 3.0
4.64 0 3.0
4.67 0 3.0
4.7 0 3.0
4.73 0 3.0
4.76 0 3.0
4.78 0 3.0
4.81 0 3.0
4.84 0 3.0
4.87 0 3.0
4.9 0 3.0
4.93 0 3.0
4.96 0 3.0
4.99 0 3.0
5.02 0 3.0
5.05 0 3.0
5.08 0 3.0
5.1 0 3.0
5.13 0 3.0
5.16 0 3.0
5.19 0 3.0
5.22 0 3.0
5.25 0 3.0
5.28 0 3.0
5.31 0 3.0
5.34 0 3.0
5.36 0 3.0
5.39 0 3.0
5.42 0 3.0
5.45 0 3.0
5.48 0 3.0
5.51 0 3.0
5.54 0 3.0
5.57 0 3.0
5.6 0 3.0
5.63 0 3.0
5.66 0 3.0
5.68 0 3.0
0.06 0.005 1.1599999999999997
0.09 0.007 1.1309999999999998
0.12 0.008 1.1019999999999999
0.15 0.01 1.073
0.17 0.012 1.0439999999999996
0.2 0.014 1.0149999999999997
0.23 0.018 0.9859999999999998
0.26 0.022 0.9569999999999999
0.29 0.027 0.9279999999999999
0.32 0.033 0.8989999999999996
0.35 0.039 0.8699999999999997
0.38 0.047 0.8409999999999997
0.41 0.058 0.8119999999999998
0.44 0.071 0.7829999999999999
0.46 0.087 0.7539999999999996
0.49 0.106 0.7249999999999996
0.52 0.127 0.6959999999999997
0.55 0.15 0.6669999999999998
0.58 0.178 0.6379999999999999
0.61 0.213 0.6089999999999995
0.64 0.26 0.5799999999999996
0.67 0.314 0.5509999999999997
0.7 0.36 0.5219999999999998
0.73 0.378 0.4929999999999999
0.75 0.382 0.46399999999999997
0.78 0.449 0.4349999999999996
0.81 0.809 0.4059999999999997
0.84 1.324 0.3769999999999998
0.87 1.275 0.34799999999999986
0.9 0.713 0.31899999999999995
0.93 0.464 0.2899999999999996
0.96 0.496 0.2609999999999997
0.99 0.487 0.23199999999999976
1.02 0.574 0.20299999999999985
1.04 0.618 0.17399999999999993
1.07 0.779 0.14499999999999957
1.1 2.212 0.11599999999999966
1.13 2.449 0.08699999999999974
1.16 1.463 0.05799999999999983
1.19 2.408 0.028999999999999915
1.22 3.267 0.0
1.25 3.159 -0.028999999999999915
0.06 0 3.0
0.09 0 3.0
0.12 0 3.0
0.15 0 3.0
0.17 0 3.0
0.2 0 3.0
0.23 0 3.0
0.26 0 3.0
0.29 0 3.0
0.32 0 3.0
0.35 0 3.0
0.38 0 3.0
0.41 0 3.0
0.44 0 3.0
0.46 0 3.0
0.49 0 3.0
0.52 0 3.0
0.55 0 3.0
0.58 0 3.0
0.61 0 3.0
0.64 0 3.0
0.67 0 3.0
0.7 0.001 3.0
0.73 0.001 3.0
0.75 0.001 3.0
0.78 0.001 3.0
0.81 0.001 3.0
0.84 0.001 3.0
0.87 0.001 3.0
0.9 0.002 3.0
0.93 0.002 3.0
0.96 0.002 3.0
0.99 0.002 3.0
1.02 0.002 3.0
1.04 0.002 3.0
1.07 0.001 3.0
1.1 0.001 3.0
1.13 0.001 3.0
1.16 0 3.0
1.19 0 3.0
1.22 0 3.0
1.25 0 3.0
1.28 0 3.0
1.31 0 3.0
1.33 0 3.0
1.36 0 3.0
1.39 0 3.0
1.42 0 3.0
1.45 0 3.0
1.48 0 3.0
1.51 0 3.0
1.54 0 3.0
1.57 0 3.0
1.6 0 3.0
1.62 0 3.0
1.65 0 3.0
1.68 0 3.0
1.71 0 3.0
1.74 0 3.0
1.77 0 3.0
1.8 0 3.0
1.83 0 3.0
1.86 0 3.0
1.89 0 3.0
1.91 0 3.0
1.94 0 3.0
1.97 0 3.0
2 0 3.0
2.03 0 3.0
2.06 0 3.0
2.09 0 3.0
2.12 0 3.0
2.15 0 3.0
2.18 0 3.0
2.2 0 3.0
2.23 0 3.0
2.26 0 3.0
2.29 0 3.0
2.32 0 3.0
2.35 0 3.0
2.38 0 3.0
2.41 0 3.0
2.44 0 3.0
2.47 0 3.0
2.49 0 3.0
2.52 0 3.0
2.55 0 3.0
2.58 0 3.0
2.61 0 3.0
2.64 0 3.0
2.67 0 3.0
2.7 0 3.0
2.73 0 3.0
2.76 0 3.0
2.78 0 3.0
2.81 0 3.0
2.84 0 3.0
2.87 0 3.0
2.9 0 3.0
2.93 0 3.0
2.96 0 3.0
2.99 0 3.0
3.02 0 3.0
3.05 0 3.0
3.07 0 3.0
3.1 0 3.0
3.13 0 3.0
3.16 0 3.0
3.19 0 3.0
3.22 0 3.0
3.25 0 3.0
3.28 0 3.0
3.31 0 3.0
3.34 0 3.0
3.36 0 3.0
3.39 0 3.0
3.42 0 3.0
3.45 0 3.0
3.48 0 3.0
3.51 0 3.0
3.54 0 3.0
3.57 0 3.0
3.6 0 3.0
3.62 0 3.0
3.65 0 3.0
3.68 0 3.0
3.71 0 3.0
3.74 0 3.0
3.77 0 3.0
3.8 0 3.0
3.83 0 3.0
3.86 0 3.0
3.89 0 3.0
3.92 0 3.0
3.94 0 3.0
3.97 0 3.0
4 0 3.0
4.03 0 3.0
4.06 0 3.0
4.09 0 3.0
4.12 0 3.0
4.15 0 3.0
4.18 0 3.0
4.2 0 3.0
4.23 0 3.0
4.26 0 3.0
4.29 0 3.0
4.32 0 3.0
4.35 0 3.0
4.38 0 3.0
4.41 0 3.0
4.44 0 3.0
4.47 0 3.0
4.5 0 3.0
4.52 0 3.0
4.55 0 3.0
4.58 0 3.0
4.61 0 3.0
4.64 0 3.0
4.67 0 3.0
4.7 0 3.0
4.73 0 3.0
4.76 0 3.0
4.78 0 3.0
4.81 0 3.0
4.84 0 3.0
4.87 0 3.0
4.9 0 3.0
4.93 0 3.0
4.96 0 3.0
4.99 0 3.0
5.02 0 3.0
5.05 0 3.0
5.08 0 3.0
5.1 0 3.0
5.13 0 3.0
5.16 0 3.0
5.19 0 3.0
5.22 0 3.0
5.25 0 3.0
5.28 0 3.0
5.31 0 3.0
5.34 0 3.0
5.36 0 3.0
5.39 0 3.0
5.42 0 3.0
5.45 0 3.0
5.48 0 3.0
5.51 0 3.0
5.54 0 3.0
5.57 0 3.0
5.6 0 3.0
5.63 0 3.0
5.66 0 3.0
5.68 0 3.0
};
\addplot [semithick, steelblue31119180, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0.003
0.09 0.004
0.12 0.005
0.15 0.006
0.17 0.007
0.2 0.009
0.23 0.011
0.26 0.013
0.29 0.017
0.32 0.021
0.35 0.025
0.38 0.03
0.41 0.036
0.44 0.044
0.46 0.054
0.49 0.067
0.52 0.081
0.55 0.097
0.58 0.116
0.61 0.138
0.64 0.167
0.67 0.204
0.7 0.245
0.73 0.285
0.75 0.316
0.78 0.332
0.81 0.345
0.84 0.407
0.87 0.659
0.9 0.992
0.93 0.862
0.96 0.573
0.99 0.454
1.02 0.422
1.04 0.48
1.07 0.526
1.1 1.906
1.13 2.133
1.16 1.116
1.19 1.619
1.22 2.102
1.25 2.152
1.28 2.172
1.31 2.271
};
\addlegendentry{38.42 N}
\addplot [semithick, darkorange25512714, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0
0.09 0
0.12 0
0.14 0
0.17 0
0.2 0
0.23 0
0.26 0
0.29 0
0.32 0
0.35 0
0.38 0
0.41 0
0.43 0
0.46 0
0.49 0
0.52 0
0.55 0
0.58 0
0.61 0
0.64 0
0.67 0
0.7 0
0.72 0
0.75 0
0.78 0
0.81 0
0.84 0
0.87 0
0.9 0
0.93 0
0.96 0
0.99 0
1.01 0
1.04 0
1.07 0
1.1 0
1.13 0
1.16 0
1.19 0
1.22 0
1.25 0
1.28 0
1.3 0
1.33 0
1.36 0
1.39 0
1.42 0
1.45 0
1.48 0
1.51 0
1.54 0
1.57 0
1.59 0
1.62 0
1.65 0
1.68 0
1.71 0
1.74 0
1.77 0
1.8 0
1.83 0
1.86 0
1.88 0
1.91 0
1.94 0
1.97 0
2 0
2.03 0
2.06 0
2.09 0
2.12 0
2.15 0
2.17 0
2.2 0
2.23 0
2.26 0
2.29 0
2.32 0
2.35 0
2.38 0
2.41 0
2.44 0
2.46 0
2.49 0
2.52 0
2.55 0
2.58 0
2.61 0
2.64 0
2.67 0
2.7 0
2.73 0
2.76 0
2.78 0
2.81 0
2.84 0
2.87 0
2.9 0
2.93 0
2.96 0
2.99 0
3.02 0
3.04 0
3.07 0
3.1 0
3.13 0
3.16 0
3.19 0
3.22 0
3.25 0
3.28 0
3.31 0
3.34 0
3.36 0
3.39 0
3.42 0
3.45 0
3.48 0
3.51 0
3.54 0
3.57 0
3.6 0
3.62 0
3.65 0
3.68 0
3.71 0
3.74 0
3.77 0
3.8 0
3.83 0
3.86 0
3.89 0
3.92 0
3.94 0
3.97 0
4 0
4.03 0
4.06 0
4.09 0
4.12 0
4.15 0
4.18 0
4.2 0
4.23 0
4.26 0
4.29 0
4.32 0
4.35 0
4.38 0
4.41 0
4.44 0
4.47 0
4.5 0
4.52 0
4.55 0
4.58 0
4.61 0
4.64 0
4.67 0
4.7 0
4.73 0
4.76 0
4.78 0
4.81 0
4.84 0
4.87 0
4.9 0
4.93 0
4.96 0
4.99 0
5.02 0
5.05 0
5.08 0
5.1 0
5.13 0
5.16 0
5.19 0
5.22 0
5.25 0
5.28 0
5.31 0
5.34 0
5.36 0
5.39 0
5.42 0
5.45 0
5.48 0
5.51 0
5.54 0
5.57 0
5.6 0
5.63 0
5.66 0
5.68 0
};
\addlegendentry{11.57 N}
\addplot [semithick, forestgreen4416044, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0
0.09 0
0.12 0
0.15 0
0.17 0
0.2 0
0.23 0
0.26 0
0.29 0
0.32 0
0.35 0
0.38 0
0.41 0
0.44 0
0.46 0
0.49 0
0.52 0
0.55 0
0.58 0
0.61 0
0.64 0
0.67 0
0.7 0
0.73 0
0.75 0
0.78 0
0.81 0
0.84 0
0.87 0
0.9 0
0.93 0
0.96 0
0.99 0
1.01 0
1.04 0
1.07 0
1.1 0
1.13 0
1.16 0
1.19 0
1.22 0
1.25 0
1.28 0
1.3 0
1.33 0
1.36 0
1.39 0
1.42 0
1.45 0
1.48 0
1.51 0
1.54 0
1.57 0
1.59 0
1.62 0
1.65 0
1.68 0
1.71 0
1.74 0
1.77 0
1.8 0
1.83 0
1.86 0
1.88 0
1.91 0
1.94 0
1.97 0
2 0
2.03 0
2.06 0
2.09 0
2.12 0
2.15 0
2.17 0
2.2 0
2.23 0
2.26 0
2.29 0
2.32 0
2.35 0
2.38 0
2.41 0
2.44 0
2.46 0
2.49 0
2.52 0
2.55 0
2.58 0
2.61 0
2.64 0
2.67 0
2.7 0
2.73 0
2.76 0
2.78 0
2.81 0
2.84 0
2.87 0
2.9 0
2.93 0
2.96 0
2.99 0
3.02 0
3.04 0
3.07 0
3.1 0
3.13 0
3.16 0
3.19 0
3.22 0
3.25 0
3.28 0
3.31 0
3.34 0
3.36 0
3.39 0
3.42 0
3.45 0
3.48 0
3.51 0
3.54 0
3.57 0
3.6 0
3.62 0
3.65 0
3.68 0
3.71 0
3.74 0
3.77 0
3.8 0
3.83 0
3.86 0
3.89 0
3.92 0
3.94 0
3.97 0
4 0
4.03 0
4.06 0
4.09 0
4.12 0
4.15 0
4.18 0
4.2 0
4.23 0
4.26 0
4.29 0
4.32 0
4.35 0
4.38 0
4.41 0
4.44 0
4.47 0
4.5 0
4.52 0
4.55 0
4.58 0
4.61 0
4.64 0
4.67 0
4.7 0
4.73 0
4.76 0
4.78 0
4.81 0
4.84 0
4.87 0
4.9 0
4.93 0
4.96 0
4.99 0
5.02 0
5.05 0
5.08 0
5.1 0
5.13 0
5.16 0
5.19 0
5.22 0
5.25 0
5.28 0
5.31 0
5.34 0
5.36 0
5.39 0
5.42 0
5.45 0
5.48 0
5.51 0
5.54 0
5.57 0
5.6 0
5.63 0
5.66 0
5.68 0
};
\addlegendentry{2.14 N}
\addplot [semithick, crimson2143940, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0.005
0.09 0.007
0.12 0.008
0.15 0.01
0.17 0.012
0.2 0.014
0.23 0.018
0.26 0.022
0.29 0.027
0.32 0.033
0.35 0.039
0.38 0.047
0.41 0.058
0.44 0.071
0.46 0.087
0.49 0.106
0.52 0.127
0.55 0.15
0.58 0.178
0.61 0.213
0.64 0.26
0.67 0.314
0.7 0.36
0.73 0.378
0.75 0.382
0.78 0.449
0.81 0.809
0.84 1.324
0.87 1.275
0.9 0.713
0.93 0.464
0.96 0.496
0.99 0.487
1.02 0.574
1.04 0.618
1.07 0.779
1.1 2.212
1.13 2.449
1.16 1.463
1.19 2.408
1.22 3.267
1.25 3.159
};
\addlegendentry{42.75 N}
\addplot [semithick, mediumpurple148103189, opacity=0.5, dash pattern=on 5.55pt off 2.4pt]
table {%
0.06 0
0.09 0
0.12 0
0.15 0
0.17 0
0.2 0
0.23 0
0.26 0
0.29 0
0.32 0
0.35 0
0.38 0
0.41 0
0.44 0
0.46 0
0.49 0
0.52 0
0.55 0
0.58 0
0.61 0
0.64 0
0.67 0
0.7 0.001
0.73 0.001
0.75 0.001
0.78 0.001
0.81 0.001
0.84 0.001
0.87 0.001
0.9 0.002
0.93 0.002
0.96 0.002
0.99 0.002
1.02 0.002
1.04 0.002
1.07 0.001
1.1 0.001
1.13 0.001
1.16 0
1.19 0
1.22 0
1.25 0
1.28 0
1.31 0
1.33 0
1.36 0
1.39 0
1.42 0
1.45 0
1.48 0
1.51 0
1.54 0
1.57 0
1.6 0
1.62 0
1.65 0
1.68 0
1.71 0
1.74 0
1.77 0
1.8 0
1.83 0
1.86 0
1.89 0
1.91 0
1.94 0
1.97 0
2 0
2.03 0
2.06 0
2.09 0
2.12 0
2.15 0
2.18 0
2.2 0
2.23 0
2.26 0
2.29 0
2.32 0
2.35 0
2.38 0
2.41 0
2.44 0
2.47 0
2.49 0
2.52 0
2.55 0
2.58 0
2.61 0
2.64 0
2.67 0
2.7 0
2.73 0
2.76 0
2.78 0
2.81 0
2.84 0
2.87 0
2.9 0
2.93 0
2.96 0
2.99 0
3.02 0
3.05 0
3.07 0
3.1 0
3.13 0
3.16 0
3.19 0
3.22 0
3.25 0
3.28 0
3.31 0
3.34 0
3.36 0
3.39 0
3.42 0
3.45 0
3.48 0
3.51 0
3.54 0
3.57 0
3.6 0
3.62 0
3.65 0
3.68 0
3.71 0
3.74 0
3.77 0
3.8 0
3.83 0
3.86 0
3.89 0
3.92 0
3.94 0
3.97 0
4 0
4.03 0
4.06 0
4.09 0
4.12 0
4.15 0
4.18 0
4.2 0
4.23 0
4.26 0
4.29 0
4.32 0
4.35 0
4.38 0
4.41 0
4.44 0
4.47 0
4.5 0
4.52 0
4.55 0
4.58 0
4.61 0
4.64 0
4.67 0
4.7 0
4.73 0
4.76 0
4.78 0
4.81 0
4.84 0
4.87 0
4.9 0
4.93 0
4.96 0
4.99 0
5.02 0
5.05 0
5.08 0
5.1 0
5.13 0
5.16 0
5.19 0
5.22 0
5.25 0
5.28 0
5.31 0
5.34 0
5.36 0
5.39 0
5.42 0
5.45 0
5.48 0
5.51 0
5.54 0
5.57 0
5.6 0
5.63 0
5.66 0
5.68 0
};
\addlegendentry{21.78 N}
\end{axis}

\end{tikzpicture}


==> sample/dacronyms.tex <==
\acronyms{

% G
\acro{GP}{Gaussian Processes}
\acro{GPSM}{Gaussian Processes semantic map}

% M
\acro{MAP}{maximum a posterior}

% S
\acro{SLAM}{simultaneous localization and mapping}

}

==> tex/abstract.tex <==
\section{Abstract}

==> tex/contributions_delete.tex <==
\section{Contributions}
Given a \textbf{desired upper bound on the false positive and false negative rate}s, our objective is to develop a fall detection algorithm for the \textbf{task of standing} that can detect potential falls caused by either \textbf{slow acting or fast acting disturbances} while \textbf{maximizing the escape (lead) time}. 

To achieve this objective, it's imperative to determine the parameters that affect the escape time, false positive rate and false negative rate. The parameters that are identified and explored in this paper are the:

\begin{itemize}
    \item Training escape time (the time when the states of a trajectory that results in a fall can start to be labeled as falling) The larger the training escape time, the less the false positive rate and escape time
    \item The fall detection method to use (clustering or classification. It's expected that clustering will perform worse when it comes to slow acting faults)
    \item Feature engineering (the features to be used, feature pre-processing,and whether or not it's better to train the detection method on each of the faults individually or together). Poor feature engineering can lead to high false positive and false negative rates and low escape time
    \item The value of $N_{monitor}$. The higher the value, the lower the escape time and false positive rate
    \item The amount of data in the window. If the window is not large enough, the escape time will decrease and the false positive and false negative rates will increase
    \item 
\end{itemize}


% This objective has different implications for the two parts that make up fall detection algorithms. 
% \begin{itemize}
%     \item \textbf{Feature Engineering} : Find the minimal set of features that can accurately differentiate between safe and falling/fallen states while maximizing the escape time
%     \item \textbf{Fall Detection algorithm}: Detect both fast and slow acting faults with sufficient escape time given a specific set of features and an upper bound on the false positive and false negative rate. 
% \end{itemize}


==> tex/feature_engineering_delete.tex <==
\section{Feature Selection}
\label{sec:feature_selection}
With the proposed algorithm achieving the desired fnr, fpr and minimum escape time across all folds, the next step is to try and improve its performance by selecting better features.  Feature selection is important as the wrong choice of features can decrease the performance of the algorithm. For instance,  using the features shown in Equation \ref{eq:features_f1_slow}

\begin{equation}
    \begin{bmatrix}
        \text{\rm knee~angle} \\
        \text{\rm hip~angle} \\
        \text{\rm vel~hip~angle} \\
        (L_{cop} + L_{com})* sgn(p_{com}^x- p_{f_\mid}^x) 
    \end{bmatrix}
    \label{eq:features_f1_slow}
\end{equation}

where $L_{cop}$ is the angular momentum about the contact point to train the SVM model on just the incipient faults with 0.9 training escape time results in 0 false positive and negative rates and an average escape time of 0.4, 0.37 and 0.38 for the training, validation, and testing sets. Whereas using the features shown in Equation \ref{eq:features_0.9_corr}
\begin{equation}
    \begin{bmatrix}
        L_{com}\\
        \text{\rm knee~angle} \\
        \text{\rm hip~angle} \\
        \text{\rm vel~knee~angle} \\
        \text{\rm vel~hip~angle} \\
        \text{\rm vel~torso} \\
        p_{com}^x - p_{cop}^x \\
        p_{com}^z- p_{f_\mid}^z
    \end{bmatrix}
    \label{eq:features_f1_slow}
\end{equation}

also results in 0 false positive and negative rates but only 0.2,0.16 and 0.18 average escape times for training, validation, and testing data. The goal of feature selection is to select features based on their redudancy and relevance. Feature selection algorithms are typically split into 3 methods, wrapper, filter and embedded methods. Wrapper methods use greedy search algorithms to add or remove features based on the chosen model's performance. Filter methods use statistical scores such as Pearson's correlation to select features. In embedded methods, feature selection is built in the chosen model. \eva{cite the following papers https://sciendo.com/article/10.2478/cait-2019-0001, https://www.frontiersin.org/articles/10.3389/fbinf.2022.927312/}. Here, we try to select features using the wrapper and filter methods. Since we are using the radial basis function kernel with our SVM classifiers, we can't explicitly compute the weight vector which would aid in determining the relevant features. \eva{cite this paper https://link.springer.com/article/10.1007/s10462-011-9205-2 } Note that there are researchers such as \eva{cite this paper https://link.springer.com/article/10.1007/s10462-011-9205-2 } who have put forward methods for feature selection for SVM with RBF kernel, however, as we are using sklearn's SVM implementation, we choose to forego embedded feature selection with the SVM classifier.  For the wrapper method we use the forward and backward sequential feature selection. The features are selected from commonly used features in literature, and are displayed in Equation \ref{eq:features_raw}. 

\begin{equation}
    \begin{bmatrix}
        L_{cop} - L_{com}\\
        L_{com} \\
        L_{cop} \\
        p_{cop}^x\\
        p_{com} \\
        v_{com} \\
        p_{com} - p_{heel} \\
        p_{toe} - p_{com}\\
        q \\
        \dot{q}\\
        p_{com} - p_{cop} \\
        (L_{cop} + L_{com})* sgn(p_{com}^x- p_{f\_mid}^x) \\
        p_{f\_mid} \\
        torso \\
        dtorso        
    \end{bmatrix}
    \label{eq:features_raw}
\end{equation}


In keeping up with the example from the beginning of this section, the SVM is trained on the selected features using the incipient and abrupt faults individually with 0.9 and 0.6 training escape times respectively. The training escape times are chosen from the first fold results in Figure \ref{fig:classifier_results} \eva{cite table when it becomes available}. 

\subsection{Distance Correlation Feature Selection}
The features are selected such that they have a correlation of greater than 0 with the escape time and less than 1 with each other. To reduce the number of features selected, the correlation thresholds can be increased and decreased respectively. The second requirement of non redundancy requires one to make a design choice between features. As a result, there are multiple features which can be derived from the same conditions. However, the performance of these resulting features can differ as can be seen in Figure \ref{fig:features_distance_corr}. As a result, this feature selection method does not give a clear cut way of selecting the features that can distinguish between our two classes. Therefore, we don't proceed to use this method with the abrupt fault trajectories. 


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/fall_detection/feature_selection/distance_corr_features.png}
    \caption{Resulting Features from Distance Correlation Feature Selection}
    \label{fig:features_distance_corr}
\end{figure}


\subsection{Sequential Feature Selection}
The sequential feature selection from sklearn is used to select the features. We got the best results by using forward featurer selection with a training escape time of 2. These features are displayed in Equation \ref{eq:features_f1_slow}. \eva{confirm how these features were found} However, when the training escape time is decreased to 0.9, the resulting features don't perform achieve as high of escape time with 0 false positive and negative rates. The results are displayed in Figure \ref{fig:features_seq_feat}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/fall_detection/feature_selection/seq_feat_selection_features.png}
    \caption{Resulting Features from Sequential Feature Selection}
    \label{fig:features_seq_feat}
\end{figure}

Even though sequential feature selection is able to find features with a higher escape time that still achieve 0 false positive and negative rate, it is time consuming. 





\section{Deep Learning}

Given the fact that feature selection is important, sequential feature selection is time consuming, and our goal of applying fall detection to more complex robots such as digit, we propose using deep neural networks such as a 1D CNN. Deep learning is capable of abstracting features from raw data. Here we take a look at the performance of a  multilayer perceptron (MLP) and 1D CNN on the fall detection data of the planar 4 link robot. The MLP and 1D CNN models used are displayed in Figure \ref{fig:mlp_model} and Figure \ref{fig:cnn_model}. Given that the fall detection problem for the planar four link robot is not complex, the neural networks perform equivalently or better than the SVM. These results are displayed in Figure   \ref{fig:neural_net_deep}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/fall_detection/feature_selection/mlp_model}
    \caption{Results from CNN and MLP}
    \label{fig:mlp_model}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/fall_detection/feature_selection/cnn_model}
    \caption{Results from CNN and MLP}
    \label{fig:cnn_model}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{img/fall_detection/feature_selection/cnn_mlp_performance.png}
    \caption{Results from CNN and MLP}
    \label{fig:neural_net_deep}
\end{figure}



==> tex/literature_review_delete.tex <==
\subsection{Literature Review}\label{sec:literature_review}
 Fall detection algorithms, however, have been implemented in some bipedal robots such as Digit \cite{ref:agility}. Most algorithms in literature tend to focus only on abrupt faults.faults is more challenging for closed loop systems due to the feedback controller's effort to mitigate the effects of the faults. \eva{cite You-jin park here}.  Generally focusing on abrupt faults does not accomplish the goal of preventing or mitigating the impact of all falls as falls can also caused by either incipient or intermittent faults. For instance, a fall detection algorithm meant for abrupt faults, might not be able to detect incipient faults 'early' enough due to the crowding phenomenon. The crowding phenomenon is the similarity between the normal and incipient faulty data which makes it difficult to separate normal data from faulty data. \eva{cite Chen et al 2020} Note that the 
 


 \eva{dive into lit review where we highlight some papers}
 
 That being said, fall detection algorithms have been implemented in some bipedal robots such as Digit\cite{ref:agility}. However, most if not all of these algorithms focus only on "fast acting" faults. As discussed in Section \ref{sec:fastSlowActingFaults} an algorithm that's trained using "fast acting" faults will still detect "slow acting" faults but with little escape time. 
 
 Escape time or lead time \cite{ref:kalyanakrishnan} is defined as the difference between the time of the actual fall and predicted fall, and is used to inform whether or not sufficient time is left for the implementation of recovery/reflexive motions. Therefore, it is important to maximize the escape time. The minimum amount of escape time needed depends on the chosen recovery algorithm and the robot dynamics. It is important to note that a large escape time can result in high false positives.
 
 False positive and false negative rates are utilized to determine the reliability of the fall detection algorithms. Threshold methods such as checking the CoM height, and orientation of the feet have been utilized to minimize the percentage of false negative rates. \cite{ref:kalyanakrishnan}.

To reduce the false positive rate the output of the fall detection algorithm is monitored for a certain number of windows ($N_{monitor}$) and a fall is declared if and only if the number of detected falls in $N_{monitor}$ is above a chosen threshold. Note that the value of $N_{monitor}$ has an inverse relationship to the false positive rate. $N_{monitor}$ and its fall detection threshold are hyperparameters. \cite{ref:kalyanakrishnan}\cite{ref:subburuman}\cite{ref:khalastchi}.


The process of designing fall detection algorithms can be divided into two parts, feature engineering and the method used for detection. The purpose of feature engineering is to choose the minimal set of features that can differentiate between the anomalous and normal data while the chosen detection method relies on the chosen features to predict falls.
 
 In literature, a combination of stability metrics such as the zero moment point(zmp)\cite{ref:zmp}, capture points/regions\cite{ref:capture_regions}, and centroidal angular momentum(L$_{\text{com}}$)\cite{ref:orin}  along with other measurements such as torso angular velocity and acceleration are utilized as features for fall detection. \footnote{ even though stability metrics are used to increase the robusteness of controllers, they individually are not a sufficient condition for falling in general cases \cite{ref:subburuman}}. There, however, isn't a systematic way of choosing the features.
 
 The fall detection methods used in literature fall into two  categories classification (feature representation)\cite{ref:park}\cite{ref:hornung}\cite{ref:hohn}\cite{ref:wu}\cite{ref:kalynakrishnan}\cite{ref:marcilino} and  nearest-neighbor (relative density)\cite{ref:khalestchi}\cite{ref:subburaman}\cite{ref:amri}\cite{ref:solar}\cite{khan}. Each of the aforementioned categories can further be classified as either shallow or deep (using neural networks), and can be used in combination with dimension reduction algorithms such as PCA \cite{ref:suetani}\cite{ref:karseen}\cite{ref:alos}.  

Classification models try to learn a model from labeled training data and then classify a data
point into one of the classes based on the learned model. A disadvantage of these algorithms is that they can output incorrect predictions if the input data is outside the training data parameters. 

Nearest-neighbor based algorithms especially those based on density assume that the normal data exist in
highly dense spaces whereas the neighborhood of anomalous data is sparse. The disadvantages of
these methods is that they tend to have high false positives if the normal instances do not exist in
dense enough neighborhoods. \cite{ml1}\cite{ml4} 
 







==> tex/problem_description_delete.tex <==
\subsection{Challenges}






As obtaining an accurate physics-based model can be time-consuming and requires explicit domain knowledge, we focus on data-driven approaches. \eva{look over this again. Need better argument for data-driven vs physics-driven}


 
 % As a result, the algorithms used for fall detection are similar to the algorithms used for anomaly detection and pattern recognition. These algorithms can either be model based or data based. Model based algorithms are good at predicting specific faults, however, they require explicit domain knowledge and can suffer from inaccuracies in the model. Data based algorithms detect faults purely from data and don't require prior knowledge of the robot. However, they are limited by the limited amount of fault data. In this paper, we'll focus on data based algorithms. Data based algorithms can be divided into several categories including classification, feature extraction, threshold-based, and clustering \eva{look into nearest-neigbor and relative density, which is how these algorithms were describe at the beginning of the paper}.  Data based algorithms can also be categorized as either shallow or deep, and supervised, semi-supervised or unsupervised. 



 
 % The overall objective of fall detection is a reliable early detection of all faults for both open and closed loop systems. Reliability in literature is determined using a combination of the following terms:  false positive rate, false negative rate, f1 score, precision, recall or sensitivity, accuracy, and area under the curve.
 
 % such as   Escape time or lead time which is defined as the difference in time from where the fault is detected to when the robot falls and the execution time of the desired reflex algorithm to determine the maximum amount of time alloted for fall detection. Given this, the larger







 % The objective is to reliably predict potential falls of bipedal robots with sufficient time  to deploy a recovery strategy. Bipedal robots are chosen because their smaller support polygon causes them to be inherently less stable in comparison to other multi-legged robots. To simplify the fall detection problem while providing a way to scale up to more complex dynamic motions such as walking, the task of standing is chosen.   

% Fall detection algorithms, in general, are a part of the robot's control system. Figure \ref{fig:fallDetector_controlSystem} depicts the fall detection algorithm's role in the robot's control system.  


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.25\textwidth]{Media/ProblemDescription/fallDetector_ControlSystemInteraction.jpg}
%     \captionsetup{font=scriptsize}
%     \caption{Interaction between the fall detector and robot's control system. The recovery strategy is embedded in the recovery controller. 
%     }
%     \label{fig:fallDetector_controlSystem}
% \end{figure}






